Building Correct SDN-Based Components from a Global Formal Mode

Software Defined Networking (SDN) brings flexibility in the construction and managment of distributed applications by reducing the constraints imposed by physical networks and by moving the control of networks closer to the applications. However mastering SDN still poses numerous challenges among which the design of correct SDN components (more specifically controller and switches). In this work we use a formal stepwise approach to model and reason on SDN. Although formal approaches have already been used in this area, this contribution is the first state-based approach; it is based on the Event-B formal method, and it enables a correct-by-construction of SDN components. We provide the steps to build, using several refinements, a global formal model of a SDN system; correct SDN components are then systematically built from the global formal model satisfying the desired properties. Event-B is used to experiment the approach.

==> eventB_nutshell.tex <==
Event-B \cite{EventB_Abrial2010,DBLP:journals/scp/HoangKBA09} is a modelling and development method where components are modelled as abstract machines which are composed and refined into concrete machines. 
An \textit{abstract machine}  describes a mathematical model of a system behaviour\footnote{A system behaviour is a discrete transition system}.
In an Event-B modelling process, abstract machines constitute the dynamic part whereas \textit{Contexts} are used to describe the static part.  
 A \textit{Context} is seen by machines. It is made of carrier sets and constants. It may contain properties (defined on the sets and constants), axioms and theorems.
A machine is made of variables and invariant, together with several \textit{event} descriptions. 
\vspace{-0.3cm}
\subsubsection*{State Space of a Machine}
The variables constrained by the invariant describe the  state space of a machine.
The change from one state to the other is due to the effect of the events of the machine. Specific properties required by the model may be included in the invariant. The predicate $I(x)$ denotes the invariant of machine, with $x$ the state variables.

\vspace{-0.3cm}
 \subsubsection*{Events of an Abstract Machine}
Within Event-B, an event is the description of a system transition. Events are  spontaneous and show the way a system evolves. 
An event $e$ is modelled as a \textit{guarded substitution}: $e \defs eG \Longrightarrow eB$ where $eG$ is the event \textit{guard} and $eB$ is the event \textit{body} or \textit{action}. The table \ref{figure:eventshape} shows the forms of generalised substitutions and their logical before-after predicate.
An event may occur only when its guard holds. 
The action of an event describes, with simultaneous generalised substitutions, how the system state evolves when this event occurs: disjoint state variables are updated simultaneously.

The effect of events are modelled with generalised logical substitution (S) using the global variables and constants. For instance a basic substitution  \texttt{x := e}  is logically equivalent to the predicate \textit{x' such that x' = e}. This is symbolically written $ x' : (x' = e)$ where $x'$ corresponds to the state variable $x$ after the substitution and $e$ is an expression. In the rest of the paper, the variable $x$ is generalised to the list of state variables.

Several events may have their guards held simultaneously; in this case, only one of them  occurs. The system makes internally a nondeterministic choice. If no guard is true the abstract system is blocking (deadlock).
%That is the substitution \texttt{x := e}  is logically equivalent to the predicate $ x' : (x' = e)$ 

\begin{table}
\begin{tabular}{|c|c|}
\hline
Event description & ~~Before-After predicate \\ 
\texttt{evt} $\defs \cdots$  & BA(x,x') $\defs \cdots$  \\
\hline
\hline
\textbf{skip} & $x' = x$ \\
\hline
\textbf{begin} $x:= S(x)$ \textbf{end} & $x' = S(x)$  \\
\hline
%The susbstitution ~$S(x)$ is logically $x' : (x' = S(x))$\\
\textbf{when} $P(x)$ \textbf{then} $x := S(x)$ \textbf{end} & $P(x) \land x'=S(x)$\\
%The substitution $S(x)$ is logically equivalent to $x : (x' =  S(x))$\\
\hline
~~\textbf{any} $lv$ \textbf{where} $P(lv, x)$ \textbf{then} $x := S(lv,x)$ \textbf{end}~~ &~~ $\exists lv.(P(bv, x) \land x'= S(lv,x)) $ \\
\hline
\end{tabular}
$~$\\
\caption{General forms of events and their before-after predicate}
\label{figure:eventshape}
\end{table}

The before-after predicate associated to each event describes it as a logical relation  between the state variables ($x$) of the model before  and after ($x'$) the occurrence of the event. This logical form of the events are used to build consistency proof obligations.

%The before-after predicate of \textsc{when}~~$P_{(x)}$ \textsc{then} ~~$S_{(x)}$ \textsc{end}  is : $P(x) \land S_a(x,x')$.

%The before-predicate of \textsc{any} $lv$ \textsc{where} $P_{(lv, x)}$ \textsc{then} ~~~~ $S_{(bv,x)}$ \textsc{end} is $\exists lv.(P(bv, x) \land S_a(lv,x)   ) $

\vspace{-0.3cm}
\subsubsection*{Semantics and Consistency}
In Event-B \textit{Proof Obligations} are defined to establish model consistency via invariant preservation. Specific properties (included in the invariant) of a system are also proved in the same way. 
%The \textit{consistency} of the model is established by such proof obligations:\\
%\textit{i)} \textit{the initialisation $U$ should establish the invariant} $I$: $~[U]I$; \\
% \textit{ii)} \textit{each event of the given abstract system should preserve the invariant of the model}. 
The proof obligation for the consistency of a model described with an invariant $I(x)$ and an event with before after predicate $BA(x,x')$ is:
$ I(x) \land BA(x,x') \implies  I(x')$.

%The proof obligation of an event with the \textsc{any} form
%(Fig. \ref{figure:eventshape}) is: $$I_{(x)} \land P_{(bv,x)}
%\land{\footnotesize \textsf{term}}(S_{(bv,x)}) \implies [S_{(bv,x)}]I_{(x)}$$
%where $I_{(x)}$ stands for the invariant of the abstract system. \\
\vspace{-0.3cm}
\subsubsection*{Refinement}
An important feature of the Event-B method is the availability of refinement technique to design concrete system from its abstract model by stepwise enrichment of the abstract model. During the refinement process new variables ($y$) are introduced; the invariant is strengthened without breaking the abstract invariant, and finally the events guards are strengthened. In the invariant $J(x,y)$ of the refinement, abstract variables ($x$) and concrete variables ($y$) are linked. The refinement is accompanied with proof obligations in order to prove their correctness with respect to the abstract model. %The proof obligation of an event with a before-after predicate $BA(x,x')$ in the abstract machine model and a before-after predicate $BAC(y,y')$ in the refined model is: $$I(x) \land J(x,y) \land BAC(y,y') \implies \exists x'.(BAA(x,x') \land J(x',y'))$$ The intuition is that a concrete event can be simulated by an abstract one.  

\vspace{-0.3cm}
\subsubsection*{Rodin Tool} The Rodin\footnote{Rodin {\small http://wiki.event-b.org/index.php/Main\_Page}} tool is an open tool dedicated to building and reasoning on B models. It is made of several modules (plug-ins) to work with B models or to interact with related tools.




==> eventB_nutshell_abstract.tex <==
Event-B \cite{EventB_Abrial2010,DBLP:journals/scp/HoangKBA09} is a modelling and development method where components are modelled as abstract machines which are composed and refined into concrete machines. 
An \textit{abstract machine}  describes a mathematical model of a system behaviour\footnote{A system behaviour is a discrete transition system}.
In an Event-B modelling process, abstract machines constitute the dynamic part whereas \textit{Contexts} are used to describe the static part.  
 A \textit{Context} is seen by machines. It is made of carrier sets and constants. It may contain properties (defined on the sets and constants), axioms and theorems.
A machine is made of variables and invariant, together with several \textit{event} descriptions. 
\textit{Proof Obligations} are defined to establish model consistency via invariant preservation. 
%Specific properties (included in the invariant) of a system are also proved in the same way. 
The Rodin\footnote{Rodin {\small http://wiki.event-b.org/index.php/Main\_Page}} tool is an open tool dedicated to building and reasoning on B models. 




